Time-of-flight estimation by utilizing Kalman filter tracking information -- Part I: the concept

Recent detector concepts at future linear or circular $e^- e^+$ colliders emphasize the benefits of time-of-flight measurements for particle identification of long-lived charged hadrons. That method relies on a precise estimation of the time-of-flight as expected, for a given mass hypothesis, from the reconstructed particle momentum and its trajectory. We show that for a realistic detector set-up, relativistic formulae are a good approximation down to lowest possible momenta. The optimally fitted track parameters are commonly defined near the interaction region. Extrapolation to a time-of-flight counter located behind the central tracking device can usually only be performed by a track model undisturbed from material effects. However, the true trajectory is distorted by multiple Coulomb scattering and the momentum is changed by energy loss. As a consequence, the estimated time-of-flight is biased by a large systematic error. This study presents a novel approach of time-of-flight estimation by splitting the trajectory into a chain of undisturbed track elements, following as close as possible the true trajectory. Each track element possesses an individual momentum $p_i$ and flight distance $l_i$. Remarkably, our formulae emerge by formally replacing the global momentum squared $p^2$ by the weighted harmonic mean of the individual $\{ p_i^2 \}$, with the weights being the corresponding individual $\{ l_i \}$. The optimally fitted parameters of the individual track elements can be obtained from track reconstruction by a Kalman filter plus smoother. However, care must be taken when including mass-dependent material effects. Explicit formulae for a simple scenario (homogeneous magnetic field and cylindrical surfaces) are given, together with an overview about the treatment of multiple Coulomb scattering and energy loss by a Kalman filter.

==> kalman.tex <==
%%%%%%%%%%%%%%%%%%
% kalman
%%%%%%%%%%%%%%%%%%

\section{Kalman filter \& smoother} 
\label{sec:kalman}

blabla

%%%%%%%%%%%%%%%%%%

==> lictoy.tex <==
%%%%%%%%%%%%%%%%%%
% part2
%%%%%%%%%%%%%%%%%%

\section{Monte Carlo study results}
\label{sec:part2}

This section is deferred ...

%%%%%%%%%%%%%%%%%%

==> tof1_bad.tex <==
%%%%%%%%%%%%%%%%%%
% tof1
%%%%%%%%%%%%%%%%%%

\section{The time-of-flight method} 
\label{sec:tof1} 

The time $T$ needed for a particle of mass $m$ moving with velocity $v$ or 
momentum $p$ along a distance $L$ in the ``laboratory frame'' is given by 
\footnote{ 
See appendix \ref{sec:app1} for definitions of the variables and the units used. } 
\begin{equation} \label{equ:2-1} 
T (m) = \frac{L}{v} = \frac{L}{\beta \, c} = 
\frac{L}{c} \cdot \sqrt{1 + \eta^{-2}} = 
\frac{L}{c} \cdot \sqrt{1 + \frac{m^2}{p^2}} 
\end{equation} 
For a relativistic particle this can be approximated as 
\begin{equation} \label{equ:2-2} 
p \gg m \quad \Longrightarrow \quad 
T (m) \approx \frac{L}{c} \cdot \left( 1 + \frac{m^2}{2 \, p^2} \right) 
\end{equation} 
\indent 
First, eqs. (\ref{equ:2-1}) and (\ref{equ:2-2}) may be used to discriminate between two 
hypotheses about a particle's mass being either $m_1$ or $m_2$. 
Let $\Delta m^2 \equiv m_2^2 - m_1^2$. 
The corresponding time-of-flight difference, as a function of both $L$ and $p$, is 
\begin{equation} \label{equ:2-3} 
\Delta T = \frac{L}{c} \cdot 
\left( \sqrt{1 + \frac{m_2^2}{p^2}} - \sqrt{1 + \frac{m_1^2}{p^2}} \: \right) 
\approx \frac{L}{2 \, c \, p^2} \cdot \Delta m^2 
\end{equation} 

Second,  precise measurement of the time-of-flight $T$ by a dedicated TOF counter, 
together with accurate estimates of the flight distance $L$ and of the momentum $p$, 
yields an estimate for the particle's mass squared, viz. 
\begin{equation} \label{equ:2-4} 
m^2 = p^2 \cdot \left[ \left( \frac{c \, T}{L} \right)^2 - 1 \right] \approx 
2 \, p^2 \cdot \left( \frac{c \, T}{L} - 1 \right) 
\end{equation} 
% Note that the approximation implies $c \, T + L \approx 2 \, L$. 
\indent 
In an ideal environment, with the errors $\sigma (p)$ and $\sigma (L)$ negligible w.r.t. 
the error $\sigma (T)$ of the measured $T$, the resulting error $\sigma (m^2)$ is  
\begin{equation} \label{equ:2-5} 
\sigma (m^2) = 2 \, p^2 \cdot \left( \frac{c \, T}{L} \right)^2 \cdot \frac{\sigma (T)}{T} 
\approx 2 \, p^2 \cdot \frac{c \, T}{L} \cdot \frac{\sigma (T)}{T} 
\end{equation} 
\indent 
Meaningful measurements of $\Delta m^2$ require 
\begin{equation} \label{equ:2-6} 
\frac{\sigma (m^2)}{\Delta m^2} \approx \frac{\sigma (T)}{\Delta T} < 1 
\end{equation} 
which, for a flight distance $L$, yields an upper limit 
\begin{equation} \label{equ:2-7} 
p^2 \approx \frac{L}{2 \, c} \cdot \frac{\Delta m^2}{\Delta T} 
< \frac{L}{2 \, c} \cdot \frac{\Delta m^2}{\sigma (T)} 
\end{equation} 

As an example, for a time resolution $\sigma(T) = 10$~ps over a flight distance 
$L = 2$~m, separation of $\pi \leftrightarrow K$ or $K \leftrightarrow p$ can in theory 
be achieved up to momenta $p < 8.65$~GeV/$c$ or 14.57~GeV/$c$, respectively. 
This only when assuming the ideal conditions mentioned above; 
in practice, the upper limits will be lower. 

Regarding eqs. (\ref{equ:2-3}) -- (\ref{equ:2-5}), the flight distance $L$ 
does not only depend on the geometry of the detector set-up, but on 
the shape of the reconstructed trajecory as well; 
hence, it is also a function of the fitted track parameters, and in particular 
of the momentum $p$. 
This dependence $L(p, \, \ldots)$ is calculated for a simple cylindrical detector set-up 
and a pure helix track model in subsection \ref{sec:tof1-1} below. 

\subsection{Discussion of a simple scenario} 
\label{sec:tof1-1}

In a detector set-up as outlined in appendix \ref{sec:app2},
% \footnote{
% Earlier versions of this appendix have been published in 
% \cite{B2C-TDR} and \cite{ Krammer}. }
the \textit{undisturbed trajectory} of a particle of unit charge and momentum $p$ 
moving in a homogeneous magnetic field of flux density $B$ is a helix 
of radius $r_H$ and slope $\cot \vartheta$: 
\begin{equation} \label{equ:2-1-1} 
r_H = \frac{p \cdot \sin \vartheta}{K_u \cdot B} \, , \qquad \qquad 
\mathrm{with} \quad K_u = 0.29979 \: \frac{\mathrm{GeV/}c}{\mathrm{T \cdot m}} 
\end{equation} 
\indent 
Assuming the particle originates at the centre point and is detected 
by a cylindrical TOF counter situated at radius $R$, its flight distance is 
\begin{equation} \label{equ:2-1-2} 
L = \frac{L_T}{\sin \vartheta} \, , \hspace{23mm} \mathrm{with} \quad 
L_T = 2 \, r_H \cdot \arcsin \frac{R}{2 \, r_H} 
\end{equation} 
being the distance projected onto the transversal plane.

Momentum $p$ and polar direction angle $\vartheta$ are known from 
track reconstruction in the CTD which is situated  in front of the TOF counter. 
If in addition coordinate $z_H$ of the hit in the TOF counter is measured 
with sufficient accuracy, 
\begin{equation} \label{equ:2-1-3} 
\cot \vartheta = \frac{z_H}{L_T} \qquad \Longrightarrow \qquad 
L = \sqrt{L_T^2 + z_H^2} 
\end{equation} 
\indent 
In order for the particle not curling back before reaching the TOF counter, 
its helix radius and its momentum must exceed a threshold 
\begin{equation} \label{equ:2-1-4} 
r_H > \frac{R}{2} \hspace{14mm} \Longrightarrow \qquad 
p > p_{min} = R \cdot \frac{K_u \cdot B}{2 \, \sin \vartheta} \, , 
\end{equation} 
hence, the projected flight distance is within $R < L_T < R \cdot \pi / 2$. 

The relative error of the transverse momentum $p_T = p \cdot \sin \vartheta$, 
estimated by a track fit, may be parametrized in the ``barrel region'' 
$| \cot \vartheta | \lesssim 1$ as 
% \cite{Krammer, Fruhwirth} 
% \begin{equation} \label{equ:2-1-5} 
% \frac{\sigma (p_T)}{p_T} = C_1 \cdot p_T \: \oplus \: \frac{C_2}{\sqrt{\sin \vartheta}} \, , 
% \end{equation} 
% i.e. 
quadratic addition of two terms, arising from detector resolution and 
multiple Coulomb scattering in CTD's material, respectively. 
The relative error of the momentum $p$, 
taking into account the correlation between $p_T$ and $\vartheta$, 
% (which can often be neglected) 
% \cite{Fruhwirth}), 
% yields \cite{Krammer, Valentan} 
% \begin{equation} \label{equ:2-1-6} 
% \frac{\sigma (p)}{p} = \sqrt{ \left( \frac{\sigma (p_T)}{p_T} \right)^2 + 
% \Big[ \, \sigma^2 (\vartheta)_{det} - \sigma^2 (\vartheta)_{m/s} \Big] 
% \cdot \cot^2 \vartheta }
% \end{equation}
% with subscripts $det$ and $m/s$ denoting the contributions from 
% detector resolution and multiple Coulomb scattering, respectively. 
% In most cases, the latter dominates \cite{Fruhwirth, Valentan} and 
may approximately be parametrized as 
% \cite{Fruhwirth} 
% \begin{equation} \label{equ:2-1-7} 
% \sigma (\vartheta)_{m/s} = \sigma (\cot \vartheta) \cdot \sin^2 \vartheta 
% \approx \frac{C_3}{p_T} \cdot \sqrt{\sin \vartheta} 
% \end{equation} 
well. Formulae are given in \cite {Krammer, Fruhwirth} and are 
thoroughly discussed in \cite{Valentan}. 

However, those error formulae qualify only globally 
% for one pre-defined reference location, 
% which is usually chosen near the centre 
% (see subsection \ref{sec:tof1-3}). 
% Therefore, they 
and are of little use for the track element approach of 
section \ref{sec:tof2} below. 
A realistic error treatment requires an adequate Monte Carlo study 
which is deferred until part II. 

\subsection{Example of calculating $\Delta T (p)$} 
\label{sec:tof1-2} 

Applied to the simple scenario of subsection \ref{sec:tof1-1}, 
% to a concrete detector set-up 
% and realistic momentum and direction resolutions, 
a numerical calculation of the time-of-flight difference $\Delta T (p)$ 
% and its error 
for $\pi^\pm \leftrightarrow K^\pm$ 
and $K^\pm \leftrightarrow p / \bar{p}$, respectively, 
is performed by using 
both the exact and the approximate formula in eq. (\ref{equ:2-3}), 
and assuming 
\begin{itemize}
\item 
a pure helix trajectory undisturbed from any material effects, 
\item 
ideal tracking resolution (zero errors on the track parameters), 
\item 
detector geometry and magnetic field of a realistic set-up \cite{ILD-IDR}: 
\begin{itemize} 
\item
$R$ = 1.80 m (inner radius of a scintillation TOF counter), 
\item 
homogeneous solenoid magnetic field of $B$ = 3.5 T. 
% \item 
% transverse momentum and polar direction angle errors, \\
% see eqs. (\ref{equ:2-1-5}) and (\ref{equ:2-1-7}), 
% are parametrized with the values \\
% $C_1 = 2 \cdot 10^{-5} / (\mathrm{GeV}/c), \: \: \: C_2 = 10^{-3}, 
% \: \: \: C_3 = 10^{-4} \, \mathrm{GeV}/c$, \footnote{ 
% The value of $C_3$ is guessed from the material budget (radiation lengths) 
% of CTD in radial direction, divided by its number of $z$ measurements, 
% as suggested in \cite{Fruhwirth}. } 
\end{itemize} 
\end{itemize} 

Results are plotted in below for momenta from $p_{min}$  
(see eq. (\ref{equ:2-1-4})) up to $p = 10$~GeV/$c$, 
and for tracks at polar angles 
$\vartheta = 90^0$ (fig. \ref{fig:2-2-1}) and 
$\vartheta = 45^0$ (fig. \ref{fig:2-2-2}). 
\begin{figure}[h!t] 
\begin{minipage}[t] 
% \centering 
\includegraphics*[width=0.75\textwidth]{deltaT_90.png} 
\caption[]{ 
$\Delta T (p)$ [ps] for polar angle $\vartheta = 90^0$; 
logarithmic ordinate.} 
% \label{fig:2-2-1} 
\end{minipage} 
\begin{minipage}[b] 
% \centering 
\includegraphics*[width=0.75\textwidth]{deltaT_45.png} 
\caption[]{ 
$\Delta T (p)$ [ps] for polar angle $\vartheta = 45^0$;
logarithmic ordinate.} 
\end{minipage} 
\caption[]{ 
TOF differences for 
$\pi \leftrightarrow K$ (purple \& red) and 
$K \leftrightarrow p$ (cyan \& blue), by the exact (red/blue solid) 
and approximate (purple/cyan dashed) formula.} 
\label{fig:2-2-2} 
\end{figure} 

In logarithmic scale and with the restriction 
$R < L \cdot \sin \vartheta < R \cdot \pi / 2$, 
the dependence of $\log L(p)$ on $p$ is very weak, and the curves follow 
approximately 
\begin{equation} 
\log_{10} \Delta T(p) \approx 
\mathrm{const} + \log_{10} \Delta m^2 - 2 \cdot \log_{10} p 
\end{equation} 
\indent 
The curves of the relativistic approximation can hardly be distinguished from 
those of the exact formula in eq. (\ref{equ:2-3}), 
even at the lowest possible momenta. 
This important feature will be essential for our novel approach in 
section \ref{sec:tof2} below. 

\subsection{Problems in realistic scenarios} 
\label{sec:tof1-3} 

The reconstruction of a charged particle track aims at an optimal estimate 
of the track's 5~parameters and $5 \cross 5$ covariance matrix 
at a pre-defined ``reference location''. 
This is achieved by an appropriate track model (imposed by the magnetic field) 
being fitted against the spatial measurements in the CTD, 
while taking into account any disturbance caused by material effects 
along the trajectory \cite{Krammer, Fruhwirth}. 

Since the fitted track parameters are input to a subsequent vertex fit, 
typical reference locations are e.g. the ``perigee point'' 
w.r.t. the centre of the beam interaction profile 
(see appendix \ref{sec:app2}) 
or the inner surface of the beam tube 
(in which case propagation to the perigee point is simple). 
Let's call this a ``type 1'' fit. 

Alternatively, a reference location may be chosen outside of the CTD, 
e.g. at the inner surface of the TOF counter, 
to be called ``type 2'' fit. 

Estimation of the time-of-flight requires either outward extrapolation of the 
fitted track from the perigee point to the TOF counter (type 1), 
or inward extrapolation in the opposite direction (type 2). 
In the conventional approach, both are realized by simply applying the 
track model to an undisturbed trajectory while ignoring all matter effects in between. 
Then, e.g. for a homogeneous magnetic field and a cylindrical TOF counter, 
the flight distance can be calculated by eqs. (\ref{equ:2-1-1})--(\ref{equ:2-1-3}). 

In reality, multiple Coulomb scattering causes stochastic kinks of the 2 
direction angles, and energy loss decreases the momentum $p$. 
Both effects modify the shape of the trajectory. 
As a result, the estimated TOF is expected to be biased by a systematic error 
growing larger with the detector's material budget increased. 

A recent simulation study, comparing type 1 and type 2 fits of 
$\pi^\pm$ and $K^\pm$ tracks in a realistic detector \cite{ILD-IDR}, 
found this bias changing sign but being less significant at type 2; 
the behaviour of $p / \bar{p}$ tracks was not conclusive \cite{Dudar}. 

This suggests defining a ``type~3'' fit as the \textit{weighted mean} 
\footnote{
Note that a weighted mean must be performed at the same reference location 
and must use the same set of parameters. 
This requires e.g. type 1 first to be propagated by the undisturbed track model 
to the reference location of type 2 (inner surface of the TOF counter).} 
of type 1 and type 2, then to use its undisturbed trajectory for the 
conventional approach of TOF estimation \cite{Regler}. 
We are, however, pursuing a more radical ansatz. 

%%%%%%%%%%%%%%%%%%
